TensorDash: Exploiting Sparsity to Accelerate Deep Neural Network Training and Inference

TensorDash is a hardware level technique for enabling data-parallel MAC units to take advantage of sparsity in their input operand streams. When used to compose a hardware accelerator for deep learning, TensorDash can speedup the training process while also increasing energy efficiency. TensorDash combines a low-cost, sparse input operand interconnect comprising an 8-input multiplexer per multiplier input, with an area-efficient hardware scheduler. While the interconnect allows a very limited set of movements per operand, the scheduler can effectively extract sparsity when it is present in the activations, weights or gradients of neural networks. Over a wide set of models covering various applications, TensorDash accelerates the training process by $1.95{\times}$ while being $1.89\times$ more energy-efficient, $1.6\times$ more energy efficient when taking on-chip and off-chip memory accesses into account. While TensorDash works with any datatype, we demonstrate it with both single-precision floating-point units and bfloat16.

==> schedulerold.tex <==
\subsubsection{Forward Propagation} 
\cref{fig:for_conv} showed the convolution of one window of the activations with each of the filters to produce one output along the channel axis of the output tensor. In this paper, we will use the term $brick$ to refer to 16 consecutive elements read along the channel axis (e.g. brick [$A_{0,0,0},...,A_{0,0,15}$]) and the term $pallet$ to refer to 16 bricks spatially consecutive along the X-axis.  As shown, our dataflow processes convolution channel first, where a activations brick is convolved with a weights brick from each filter to produce one partial sum in each output activations channel. 

Considering an accelerator with a tile configuration of 16 rows by 16 columns of processing elements (PE), where each row has a weights brick to be reused with an activations brick provided for each column. Each PE can multiply and accumulate a brick of activations and weight pairs. Our dataflow reads an activations pallet from memory along with 16 weights bricks each from a different filter. The tile produces 256 partial sums in the form of an output pallet.

Processing the fully-connected layers proceeds in a similar manner.

\subsubsection{Back Propagation: Input Gradients} 

For convolutional layers and as Fig.\cref{fig:inGrad_conv} shows we convolve each activation pallet with 16 weight bricks each from a different reshaped filter. 

For fully-connected layers we use the same dataflow used as in the forward pass is used in calculating activation gradients in the backward pass.

\subsubsection{Back Propagation: Weight Gradients}
dataflow?????

\subsection{Static vs. Dynamic Sparsity}
The software-based front-end of Tactical works well for static sparsity such as model sparsity where the weights that are equal to zero already known before execution. The front-end then takes the model parameters as input and reschedules them taking into account the hardware-supported connectivity in order to minimize the ineffectual operations at run-time. The rescheduling then is a one-time process that is done only once per model.
However, this software-based scheduling leaves considerable amount of dynamic sparsity untapped. Dynamic sparsity appears dynamically at run-time including: 1) activations sparsity during inference, and 2) activations and gradients sparsity during training. To exploit dynamic sparsity, an accelerator needs a hardware scheduler that takes as input the values, would it be activations or gradients, and moves them in space and time according to the connectivity supported in the compute unit. Along with the shuffled values, the hardware scheduler generates a schedule that will drive the connections in the compute unit when the values are brought for processing by the next layer.



\section{DNN Training}
Considering our accelerator tile configuration, the dataflow supplies one column of PEs with an activation brick each is reused with 16 weights brick each supplied to one row of PEs resulting in 16 different partial sums.



\section{Dynamic Tactical} 
\label{sec:dtactical}

\subsection{Dynamic Scheduler}

Dynamically generating the schedule for the sparse values can be done either on the input side of a layer or at the output side of the previous layer while generating those values. Both approaches can be implemented with low hardware overhead compared to the compute logic and the on-chip memory. However, the second approach has an advantage since it serves also as a compression technique where the output values will be compactly packed with less zero values. The approach is feasible since generating the next set of output values would typically take tens to thousands of cycles which allows enough time for the current set of values to be rescheduled meanwhile. 

Following the second approach, we describe an implementation of a hardware scheduler that can be attached to the output of the compute unit to pre-schedule the values as they come out preparing them for the next layer. While our proposed scheduler is generic enough to accommodate any of the proposed <ahead, aside> configurations, in the example below we assume a $T\langle2,5\rangle$ configuration where the scheduler considers two ahead sets of values. As shown in \cref{fig:promo_map}, to fill a sparse slot like $Curr_{12}$, it can promote one of 7 possible candidate values; two from the same slot but ahead in time (shown in orange) and five from the neighboring slots in the ahead sets (shown in blue).

The scheduler buffers three successive chunks of the output values: 1) Curr: the earliest chunk among the three and which is being scheduled at the moment, 2) Ah1: the first ahead chunk that comes right after Curr, and 3) Ah2: the second ahead chunk and the most recent among the three. The chunk length is the number of output values concurrently processed by the compute unit. In the example implementation shown we assume the length is 16. The example implementation shown takes 16 cycles to finish the scheduling of the Curr chunk by performing the necessary promotion, if needed, from Ah1 and Ah2 for one Curr position at a time. However, it is possible to finish the scheduling in less cycles by concurrently processing those positions in Curr that have non-overlapping promotion candidates in Ah1 and Ah2. For example, the purple and green positions in \cref{fig:promo_map} can be used to fill the sparse slot $Curr_6$ in parallel with processing slot $Curr_12$. A more complex parallel implementation would be able to process positions with overlapping candidates by having a conflict resolver that prioritize one position over the other in case of a conflict.

\begin{figure}%                 
                \centering
                \includegraphics[width=0.35\textwidth]{figures/curr_effect.pdf}
                \caption{Curr registers holding the chunk of values being scheduled. Effectual elements are detected.}
                \label{fig:curr_effect}
\end{figure}

\begin{figure}%                 
                \centering
                \includegraphics[width=0.35\textwidth]{figures/ah1_2_effect.pdf}
                \caption{Ah1 and Ah2 registers holding promotion candidates. Effectual elements are detected.}
                \label{fig:ah1_2_effect}
\end{figure}

The implementation is detailed in \cref{fig:curr_effect} to . As shown in \cref{fig:curr_effect} and \cref{fig:ah1_2_effect}, three sets of 16 registers are used to buffer the Curr, Ah1 and Ah2 chunks highlighted in red, green and blue respectively. Those are parallel loaded with the current chunk to be scheduled and the two ahead chunks to promote from. Then, all the values go through comparators ``$\neq 0$'' to detect the effectual values. For the Curr chunk this helps distinguishing the positions that need promotion while for Ah1 and Ah2 this identifies the candidates that can be used to fill the ineffectual positions in Curr. The outputs of the comparators are [$Curr\_Effec_{15}$ ... $Curr\_Effec_0$], [$Ah1\_Effec_{15}$ ... $Ah1\_Effec_0$] and [$Ah2\_Effec_{15}$ ... $Ah2\_Effec_0$]. 

\begin{figure}%                 
                \centering
                \includegraphics[width=0.4\textwidth]{figures/candidate_counters2.pdf}
                \caption{Candidate counters prioritize the position with the least number of effectual candidates.}
                \label{fig:candidate_counters}
\end{figure}

\begin{figure}%                 
                \centering
                \includegraphics[width=0.30\textwidth]{figures/priority_encoders.pdf}
                \caption{Priority encoders prioritize the candidates per position. $isMinPos_i$ decides which position to promote for.}
                \label{fig:priority_encoders}
\end{figure}
These three vectors are then used to drive 16 candidate counters [$Count\_Candid_{15}$ ... $Count\_Candid_0$], shown in \cref{fig:candidate_counters}, and 16 priority encoders [$Priority\_Enc_{15}$ ... $Priority\_Enc_0$], shown in \cref{fig:priority_encoders}. Each candidate counter and priority encoder correspond to one position in Curr. A priority encoder $Priority\_Enc_i$ prioritizes the effectual candidates corresponding to position i in a predetermined order such as the one shown in \cref{fig:promotion_priority_map} where a lower number means higher priority. It is necessary to give the highest priority to the original value in Curr if it is effectual, i.e. the highest priority is given to $Curr\_Effec_i$. This is to ensure no promotion will happen if the position contains an effectual value. For each position I, the corresponding priority encoder $Priority\_Enc_i$ outputs the index of the effectual candidate with the highest priority $Promo\_selec_i$. The indices [$Promo\_selec_{15}$ ... $Promo\_selec_0$] drive the selection lines of the 16 8-to-1 multiplexers, shown in blue, selecting the highest priority candidate per Curr position.

\begin{figure}%                 
                \centering
                \includegraphics[width=0.35\textwidth]{figures/promotion_priority_map.png}
                \caption{Example priority order of the promotion candidates.}
                \label{fig:promotion_priority_map}
\end{figure}

Meanwhile, a candidate counter $Count\_Candid_i$ counts how many effectual candidates are available for position i to promote from. Thus, $Count\_Candid_i$ takes 7 candidate inputs, 4 from [$Ah1\_Effec_{15}$ ... $Ah1\_Effec_0$] and 3 from [$Ah2\_Effec_{15}$ ... $Ah2\_Effec_0$], renamed as [$Cand\_Effec_{i,7}$ ... $Cand\_Effec_{i,1}$]. We use 16 1-bit registers [$Done_{15}$ ... $Done_0$] to keep track of the positions that have already been processed. Each $Done_i$ register is concatenated as a \textit{most significant bit} to the output of the corresponding candidate counter. Thus, a position that has been already processed will appear as if it has at least 8 candidates effectively excluding that position from competing again for a promotion. The number of candidates per position are then fed into a minimum tree that finds the position with the minimum number of candidates $PosIdx_{minCand}$. That position will receive the highest priority to be processed first otherwise it will likely have no effectual candidates left. $PosIdx_{minCand}$ then goes through a decoder to produce a 1-hot vector [$isMinPos_{15}$ ... $isMinPos_0$] where only the bit corresponding to the position j selected for processing, e.g. $isMinPos_j$, is set. That bit then affects three registers: 1) $Done_j$: to mark position j as ``processed'', 2) $Curr_j$: to enable writing the promoted value to the corresponding Curr position, and 3) $Sched_j$: to enable writing the index of the highest priority effectual candidate $Promo\_selec_j$ to the corresponding Sched register, shown in \cref{fig:priority_encoders}.


\begin{figure}%                 
                \centering
                \includegraphics[width=0.48\textwidth]{figures/Ah_reset.pdf}
                \caption{$Ah1\_rst_0$ and $Ah2\_rst_0$ driving the reset signal of $Ah1_0$ and $Ah2_0$ respectively.}
                \label{fig:Ah_reset}
\end{figure}
The final step is to reset the promoted value in Ah1 or Ah2 to zero indicating that the value has been moved to the processed Curr position. It can be inferred from \cref{fig:promotion_priority_map} that a register $Ah1_i$ is a promotion candidate for 4 Curr positions: i, i-1, i+1, and i-3. Similarly, a register $Ah2_i$ is a promotion candidate for 3 Curr positions: i, i-2, and i+2. Thus, considering the priority order of the promotion candidates shown in \cref{fig:promotion_priority_map}, the reset signal for $Ah1_i$ and $Ah2_i$ can be driven by the following expressions respectively:
\begin{eqnarray*}\label{eq:ah1reset} 
Ah1\_rst_i & = &(isMinPos_{i\ \ }\   \& (Promo\_selec_{i\ }\ == 1)) | \\
		 & &    (isMinPos_{i-1}      \& (Promo\_selec_{i-1} == 4)) | \\
		 & &    (isMinPos_{i+1}      \& (Promo\_selec_{i+1} == 3)) | \\
		 & &    (isMinPos_{i-3}      \& (Promo\_selec_{i-3} == 5)) 
\end{eqnarray*}
\begin{eqnarray*}\label{eq:ah2reset}
Ah2\_rst_i & = &(isMinPos_{i\ \ }\   \& (Promo_selec_{i\ }\ == 2)) | \\
		 & &    (isMinPos_{i-2}      \& (Promo_selec_{i-2} == 7)) | \\
		 & &    (isMinPos_{i+2}      \& (Promo_selec_{i+2} == 6)) | \\
\end{eqnarray*}



Where the position indices i-1, i+1, i-3, i-2, i+2 are modulus 16 to wrap around on the edges of the vectors. For example, the $Ah1\_rst_0$ and $Ah2\_rst_0$ are shown in \cref{fig:Ah_reset}.

The outputs of the dynamic scheduler after 16 cycles are: 1) [$Curr_{15}$ ... $Curr_0$]: where the possible promotions were made from [$Ah1_{15}$ ... $Ah1_0$] and [$Ah2_{15}$ ... $Ah2_0$], and 2) [$Sched_{15}$ ... $Sched_0$]: containing the schedule generated according to the promotions performed. Then, the roles of Curr, Ah1 and Ah2 are rotated where Ah1 becomes the new Curr, Ah2 becomes Ah1, and the next output chunk calculated by the processing unit can be loaded into Curr which becomes Ah2.


\subsection{Tile Organization}


\subsection{Memory System}

\subsection{Handling Strides}

==> training.tex <==
\subsection{Forward Propagation} 
\subsubsection{Convolution Layers}
To get the output activations of the next layer, a 3D convolution is performed between the input activations and each of the weight filers to produce one channel in the output activations: 

\begin{equation} \label{eq:for_conv}
    A^{S/i+1}_{oc,ox,oy} = \sum^{C}_{ci=0} \sum^{Kx}_{xi=0} \sum^{Ky}_{yi=0} A^{S/i}_{ci,ox+s*xi,oy*s+yi} * W^{i/oc}_{ci,xi,yi}
\end{equation}

 where $s$ is the layer convolution stride.
 
\cref{fig:for_conv} shows the convolution of one window in the activations with each of the weight filters to produce one output in each channel output activations. In this paper, we will use the term $brick$ to refer to 16 consecutive elements read channel first (e.g. brick [$A_{0,0,0},...,A_{0,0,15}$]) and the term $pallet$ to refer to 16 spatially consecutive bricks.  As shown, our dataflow processes convolution channel first, where a activations brick is convolved with a weights brick from each filter to produce one partial sum in each output activations channel. \par
Considering an accelerator with a tile configuration of 16 rows by 16 columns of processing elements (PE), where each row has a weights brick to be reused with an activations brick provided for each column. Each PE can multiply and accumulate a brick of activations and weight pairs. Our dataflow reads an activations pallet from memory along with 16 weights bricks each from a different filter. The tile produces 256 partial sums in the form of an output pallet.

\begin{figure}                
\centering
\includegraphics[scale=0.2]{figures/training_summary.png}
\caption{Computations during forward and backward phases of training}
\label{fig:training_summary}
\end{figure}


\begin{figure}                
\centering
\includegraphics[width=0.47\textwidth]{figures/for_conv.png}
\caption{Forward convolution of one training sample}
\label{fig:for_conv}
\end{figure}

\subsubsection{Fully Connected Layers}
Each output activations in fully connected layers is calculated as in equation \ref{eq:for_fc}.

\begin{equation} \label{eq:for_fc}
    A^{S/i+1}_{oc} = \sum^{C}_{ci=0} A^{S/i}_{ci} * W^{i,oc}_{ci}
\end{equation}

\subsection{Back Propagation: Input Gradients} 
In the backward pass, the weights per layer are updated according to the activation gradients. Hence, back-propagation involves two simultaneous convolutions: one to propagate the activations gradients between layers, and the other to calculate the weight gradients of each layer.

\begin{figure}             
\centering
\includegraphics[width=0.47\textwidth]{figures/inGrad_conv.png}
\caption{Calculating input gradients of one training sample.}
\label{fig:inGrad_conv}
\end{figure}

\subsubsection{Convolution Layers}
To calculate the activation gradients of one layer, a 3D convolution is performed between a reshaped version of the filters with the activation gradients of the subsequent layer. The filters are reconstructed channel-wise and rotated by 180 degrees before the convolution as shown in equation \cref{eq:inGrad_conv} and Fig.\cref{fig:inGrad_conv}, where the activation gradients are dilated according to the convolution stride of the layer.

\begin{equation} \label{eq:inGrad_conv}
    G^{S/i-1}_{oc,ox,oy} = \sum^{F}_{ci=0} \sum^{Kx}_{xi=0} \sum^{Ky}_{yi=0} G^{S/i}_{ci,ox+xi,oy+yi} * {W_{rotated}}^{i,ci}_{oc,xi,yi}
\end{equation}

Our dataflow convolves each activation pallet with 16 weight bricks each from a different reshaped filter. 

\subsubsection{Fully Connected Layers}
Each input activation gradient is calculated as described in equation \cref{eq:inGrad_fc}.

\begin{equation} \label{eq:inGrad_fc}
    G^{S/i-1}_{oc} = \sum^{C}_{ci=0} G^{S/i}_{ci} * W^{i,ci}_{oc}
\end{equation}

The same dataflow used in processing fully-connected layers in the forward pass is used in calculating activation gradients in the backward pass.

\subsection{Back Propagation: Weight Gradients}
The weight gradients that are calculated per layer are accumulated across the training samples within a mini-batch and then used to update the network parameters as described in Equation \cref{eq:weight_update}, where $i$ is the weight number, $t$ is the epoch number, $\alpha$ is the learning rate, and $S$ is the mini-batch size.

\begin{equation} \label{eq:weight_update}
    W^{i}_{t+1} = W^{i}_{t} - \alpha * \sum^{S}_{s=0} G_{s}/S
\end{equation}

\subsubsection{Convolution Layers}
The weight gradients of the filters are calculated as a 2D convolution between the input activation of each training sample with its corresponding output gradients as described in Equation \cref{eq:weightGrad_conv} and Fig. \ref{fig:back_conv_weightGrad}. Similar to calculating input gradients, the activation gradients are dilated according to the stride.

\begin{equation} \label{eq:weightGrad_conv}
    Gw^{i,f}_{oc,ox,oy} = \sum^{S}_{si=0} \sum^{Nox}_{xi=0} \sum^{Noy}_{yi=0} G^{si/i}_{f,xi,yi}
\end{equation}

\begin{figure}             
\centering
\includegraphics[width=0.47\textwidth]{figures/weightGrad_conv.png}
\caption{Calculating weight gradients for one training sample}
\label{fig:back_conv_weightGrad}
\end{figure}

\subsubsection{Fully-Connected Layers}
Since in fully-connected layers each weight sees only one input activation and contributes to only one output activation, each weight gradient is only a scalar product between the input activation and the output activation it affects as described in equation \cref{eq:weightGrad_fc}.

\begin{equation} \label{eq:weightGrad_fc}
    Gw^{i,f}_{oc} = G^{S/i}_{f} * A^{S/i}_{oc}
\end{equation}
